Molecular Property Prediction: A Multilevel Quantum Interactions Modeling Perspective

Predicting molecular properties (e.g., atomization energy) is an essential issue in quantum chemistry, which could speed up much research progress, such as drug designing and substance discovery. Traditional studies based on density functional theory (DFT) in physics are proved to be time-consuming for predicting large number of molecules. Recently, the machine learning methods, which consider much rule-based information, have also shown potentials for this issue. However, the complex inherent quantum interactions of molecules are still largely underexplored by existing solutions. In this paper, we propose a generalizable and transferable Multilevel Graph Convolutional neural Network (MGCN) for molecular property prediction. Specifically, we represent each molecule as a graph to preserve its internal structure. Moreover, the well-designed hierarchical graph neural network directly extracts features from the conformation and spatial information followed by the multilevel interactions. As a consequence, the multilevel overall representations can be utilized to make the prediction. Extensive experiments on both datasets of equilibrium and off-equilibrium molecules demonstrate the effectiveness of our model. Furthermore, the detailed results also prove that MGCN is generalizable and transferable for the prediction.

==> 1_abstract.tex <==
\begin{abstract}
Predicting molecular properties (e.g., atomization energy) is an essential issue in quantum chemistry, which could speed up much research progress, such as drug designing and substance discovery. Traditional studies based on density functional theory (DFT) in physics are proved to be time-consuming for predicting large number of molecules. Recently, the machine learning methods, which consider much rule-based information, have also shown potentials for this issue. However, the complex inherent quantum interactions of molecules are still largely underexplored by existing solutions. In this paper, we propose a generalizable and transferable Multilevel Graph Convolutional neural Network (MGCN) for molecular property prediction. Specifically, we represent each molecule as a graph to preserve its internal structure. Moreover, the well-designed hierarchical graph neural network directly extracts features from the conformation and spatial information followed by the multilevel interactions. As a consequence, the multilevel overall representations can be utilized to make the prediction. Extensive experiments on both datasets of equilibrium and off-equilibrium molecules demonstrate the effectiveness of our model. Furthermore, the detailed results also prove that MGCN is generalizable and transferable for the prediction.
\end{abstract}





==> 2_introduction.tex <==

\section{Introduction}
Predicting molecular properties, such as atomization energy, is one of the fundamental issues in quantum chemical science.
Indeed, it has attracted much attention in relevant fields of physics, chemistry and computer science, since it speeds up the societal and technological progress in the application of discovering substances with desired characteristics, such as drug design with specific target and new material manufacture~\cite{becke2007quantum,oglic2017active}.

%From drug development to energy production, the discovery of molecules with desired characteristics can make substantial societal and technological progress \cite{becke2007quantum,oglic2017active}. An efficient approach to predict molecular properties will tremendously speed up the process because many discoveries can be guided by screening a large space of potential molecules. For instance, the prediction of atomization energy at 0K (the property $U0$ in Figure \ref{demo}.d) could help the discovery of stable molecules. Therefore, molecular property prediction has drawn great attention. In a molecular system, the quantum interactions between particles create quantum correlations and entanglement that are closely related to molecular properties \cite{thouless2014quantum}. Consequently， modeling these interactions is a crucial part of the prediction. 



% In the past decade, molecular property prediction has attracted people with multidisciplinary interests. Because an efficient approach to make the prediction will tremendously speed up the discovery of molecules with desired properties by exploring the given molecular space. Consequently, it will benefit material informatics, medicine designing, and food development . A crucial part of the prediction task is modeling the quantum interactions in molecules, which aims at discovering the latent representation of atoms \cite{jin2018junction,GmezBombarelli2018AutomaticCD}. Massive efforts have been made to the solutions.

In the literature, density functional theory (DFT) plays an important role in physics for molecular property prediction. It holds a common statement that the quantum interactions between particles (e.g., atom) create the correlation and entanglement of molecules which are closely related to their inherent properties~\cite{thouless2014quantum}. Along this line, many quantum mechanical methods based on DFT have been developed to model the quantum interactions of molecules for the prediction~\cite{hohenberg1964inhomogeneous,kohn1965self}. However, DFTs are computationally costly since they usually use specific functions to determine the interactions of particles, which proves to be extraordinarily time consuming. For example, experimental results indicated that it took nearly an hour to predict the properties of merely one molecule with 20 atoms~\cite{Gilmer2017NeuralMP}. Obviously, it is unacceptable to make prediction on large number of molecules in chemical compound space. Therefore, it is necessary to find more effective solutions. 

\begin{figure}[tb]
	\centerline{\includegraphics[width=8.5cm]{figures/demo} }
	\caption{Illustration of the process of a molecule (\ce{CH2O2}) via our method.}
	\label{demo}
\end{figure}

%Quantum mechanical methods based on density functional theory (DFT) \cite{hohenberg1964inhomogeneous,kohn1965self} are very popular models to make the prediction. These model hide the complexity of the task by mapping the quantum interactions onto every single particle. However, DFT based approaches are extraordinarily time-consuming so that it is hard to make an exhaustive exploration in chemical compound space with this model. Recently, due to the remarkable success that Machine Learning (ML) have achieved in a large number of tasks including natural language processing and computer vision \cite{Karpathy2014LargeScaleVC,He2016DeepRL}, many pioneering efforts have been committed to the research of solving the problem with data-driven methods \cite{faber2017prediction,schutt2017schnet}. Although prior works had developed some accurate ML models, the limitations of these approaches and unresolved challenges of the task make the young filed still pretty much open.

% However, the traditional CNNs typically work on the data with an underlying Euclidean or grid-like structure while the molecules are naturally presented as graphs (see the second part of Figure  \ref{demo}). Therefore, some previous approaches utilized the extended CNNs to make the chemical prediction. These models \cite{schutt2017schnet,li2015gated,schutt2017quantum,Gilmer2017NeuralMP} learn the representations of a molecule by blending the interaction between atoms together and do not model the interactions at multiple levels, e.g., pair-wise and triple wise influence. Thus, these representations are not generalizable adequately.

Recently, inspired by the remarkable success of machine learning in many tasks including computer vision and natural language processing~\cite{Karpathy2014LargeScaleVC,He2016DeepRL,ren2015faster}, researchers have shown the potentials of these data-driven techniques for molecular property prediction~\cite{faber2017prediction,schutt2017schnet}. Generally, these studies mainly rely on rule-based feature engineering (e.g., bag of atom bonds) or treat molecules as grid-like structures (e.g., 2D images or text). However, few of them directly take the inherent quantum interactions of molecules into consideration, causing severe information loss, which makes the molecular property prediction problem pretty much open.

Unfortunately, there are many technical and domain challenges along this line. First, there are highly complex quantum interactions, such as distracted attraction, exchange repulsion and electrostatic interaction in molecules, especially in the large molecules~\cite{kollman1985theory}. It is hard to model them with analytical methods. Second, compared with traditional tasks including computer vision, the amount of labeled molecule data is significantly limited, which requires a generalizable approach for the prediction. Last but not least, in practice, we are often provided with labeled data of small and medium molecules except large molecules since the calculation of them are expensive. Thus, it is necessary to notice this unbalancedness to propose a transferable solution for property prediction of large molecules using the model trained on smaller ones.

%There are many tough challenges associated with the prediction of molecular properties. The first problem is that the quantum interactions in molecules are highly complex, especially in the large molecules \cite{kollman1985theory}. These interactions include distracted attraction, exchange repulsion, electrostatic interaction, etc. Therefore, it is hard to model them with analytical methods. The second challenge is that existing datasets are not large sufficiently comparing with the entire chemical space. The lack of data demands that the model should be generalizable while the previous models can barely meet the requirement. The last probelm is that, most data in existing datasets are small and medium molecules and few of them are large molecules owing to the expensive calculations. Under the circumstance, a satisfying approach is ought to be transferable to tackle the unbalanced distribution. However, few of previous arts concentrated on the generalizability and transferability of models.

To address these challenges, in this paper, we propose a well-designed Multilevel Graph Convolutional Neural Network (MGCN) for predicting properties of molecules by directly incorporating their quantum interactions. Figure ~\ref{demo} demonstrates the process of our approach. Specifically, we first represent each molecule as an interaction graph, which could preserve its internal structure without information loss. Then we propose a hierarchical graph convolutional neural network to model the multilevel quantum interactions based on the graph-like molecular structures. Here, we follow  the DFT theory that the quantum interactions could be transformed at different levels, i.e., atom-wise refers to the inherent influence of each atom (e.g., oxygen), atom-pair refers to the interaction between two atoms, atom-triple means the correlation among three atoms, and so on. Thus, our proposed graph network incorporates hierarchical layers of point-wise, pair-wise, triple-wise, etc to extract representations of the multilevel interactions, respectively. Finally, the overall interaction representation from all levels could be utilized to make the property prediction. We conduct extensive experiments on both datasets of equilibrium and off-equilibrium molecules, where the experimental results shows the effectiveness of our proposed approach. Moreover, as MGCN could naturally pass the interaction information of molecules level by level, which also proves the superior ability of generalizability and transferability.


%To address these challenges, we propose the Multiscale Graph Convolutional Neural Network (MGCN). Because molecules are naturally presented as graphs without the loss of information (Fig\ref{demo}.$a$, 1.$b$), we choose the graph-like data as our input instead of other grid-like format. Then, we utilize the inherent multilevel structure of molecular system to model the quantum interactions. Figure \ref{demo}.c demonstrates the progress, the first-order representations are atom embeddings (noted with $\alpha$) that only consider the property of isolated atoms. In the next phase, a well-designed interaction layer take atom embeddings and edge information as input to generate the pair-wise interaction representations (noted with $beta$). The descriptors at deep level are generated in the same way. We model the multilevel interactions respectively to avoid the complexity of learning the complicated interactions in a combined representation directly. Furthermore, the abundant information of conformation and structure is learned in the representations rather than vanishing in blending. Thus, our model is more generalizable than previous works benefiting from the robust features extracted by the multiscale interaction layers. Besides, pre-trained atom and edge embeddings could be used as the initialization of other models. That enhances the ability of transfering the knowledge learned from smaller moleucles to larger molecules. However, few of prior arts concentrated on the generalizability and transferability of models.


% Considering the interaction graph and multiscale interactions demonstrated in Figure  \ref{demo}, the first-order smooth latent representations are atom embeddings (noted with $\alpha$). Then, we design an interaction layer to generate the representations of deeper level by blending the former node and edge des   criptors. For instance, the representations of pair-wise interactions (see Figure  \ref{demo}, noted with $\beta$) are the output of the first interaction layer with atom embeddings as input. The spatial information that represented as the distance tensor is also involved in modeling different level interactions. The features we learnt will be fed into a two-layer neural network to get the final prediction taking account of the additivity and locality of the molecular system. The final target to predict are important properties of molecules, such as the atomization energy at 0K ($U0$ in Figure  \ref{demo}). The hierarchical structure models the pair-wise, triple-wise and deeper interactions respectively rather than learning the complicated interactions in the combined representation directly. Benefiting from the abundant information of conformation and structures that passed by interaction layers, our approach attains the better performance than baselines. Furthermore, the experimental results show that MGCN is capable of transferring the knowledge learned from smaller molecules to larger molecules. 

%The key contributions of our study are summarized as following: We develop the MGCN model to predict novel molecular properties and this method shows the state-of-the-art performance. This CNN-like model which takes the graph-structured molecular data as input are more generalizable and transferable than former approaches owing to the multiscale quantum interaction modeling. Several experiments in two pervalent datasets proved the competency of our model. Moreover, numerical results shows that our model spends much less time than the classic DFT methods to make prediction. 


% \begin{itemize}
%     \item We develop the MGCN model: an CNN model which could directly be performed on graph-like data of arbitrary size. MGCN shows the state of the art performance in two different datasets. Otherwise, once the training is completed, MGCN spends much less time than the DFT methods to infer the results.  
%     \item We introduce an approach to model the multiscale quantum interactions in the MGCN. By this way, the representations we learned in the network satisfy several significant desirable properties, such as translation invariance, rotation invariance, index invariance, size extensive. More importantly, the experiments prove that the representations are transferable and generalizable as well.
% \end{itemize}







==> 3_related_work.tex <==
\section{Related work}
Generally, the related work of our research could be classified into the following three categories.

\textbf{Density Functional Theory.}
Molecular property prediction problem has been studied for a long time in physics, chemistry and material science~\cite{wang2011application}. In the literature, density functional theory (DFT) is the most popular method, which plays a vital role in making the prediction, and could date back to 1960s~\cite{hohenberg1964inhomogeneous,kohn1965self,lawless2002information}. Generally, it states that the quantum interactions between particles (e.g., atoms) create the correlation and entanglement of molecules which are closely related to their inherent properties~\cite{thouless2014quantum}. Following this theory, many DFT based methods, such as B3LYP, were proposed, which mapped the quantum interactions of molecules onto every single particles, for predicting the properties~\cite{yanai2004new}. However, the complexity of DFT could be approximated as $\mathcal{O}(N^3)$, where $N$ denotes the number of particles. Therefore, it is time-consuming in the experiments and unacceptable for the prediction when facing large number of molecules~\cite{Gilmer2017NeuralMP}.

%\textbf{Density Functional Theory.}\ The density functional theory (DFT) \cite{hohenberg1964inhomogeneous,kohn1965self,lawless2002information} based method is a widely used quantum mechanical approach to predict the properties of molecules. However, DFT is extraordinarily time-consuming \cite{Gilmer2017NeuralMP}. Thus, many competent data-driven models emerged, and we will introduce these work in this section.
% TODO 加一句为啥DFT很慢  

\textbf{Traditional Machine Learning Methods.}
To find more efficient solutions for molecular property prediction, researchers have attempted to leverage various machine learning models, such as kernel ridge regression, random forest and Elastic Net \cite{faber2017prediction,zou2005regularization}. Generally, they rely on rule-based hand crafted features using the domain knowledge of physics and chemistry, including bag of bonds, coulomb matrix, and histogram of distances, angles and dihedral angles~\cite{huang2016communication,hansen2015machine,montavon2012learning}. Although some superior experimental results have been achieved, these traditional machine learning methods take manual feature engineering, which requires much domain expertise. Thus, they are often restricted in practice.

%\textbf{Traditional Machine Learning Models.}\ Machine learning (ML) models were proved to be more efficient and accurate than original DFT based methods in small organic molecules \cite{faber2017prediction}. Many hand-craft features, such as bag of bonds (BoB), Bonds-angle machine learning (BAML), and Histogram of distances, angles and dihedral angles (HDAD), were developed to feed to some machine learning methods like Kernel Ridge Regression (KRR), Random Forest (RF) \cite{hansen2015machine,huang2016communication}. \citeauthor{faber2017prediction} benchmarked many combinations of representations and ML methods, and the statistical evidence suggests KRR has the best performance across most prediction tasks \cite{faber2017prediction}. 

%Although some of these traditional regressors lead to lowest out-of-sample error in a few target properties, their performance highly depends on the manual feature engineering. Therefore, these models require domain expertise to hand design feature extractors.

\textbf{Deep Neural Networks.}
Compared to traditional machine learning models, deep neural networks hold a superiority of automatic feature learning, which have achieved great success in many applications, such as speech recognition~\cite{zhu2016co}, computer vision~\cite{lecun1995convolutional} and natural language processing~\cite{collobert2008unified}. With this ability, researchers have noticed the potentials of these deep methods for molecular property prediction. Along this line, convolutional neural network based models were proposed, where they represented each molecule as grid-like structures, such as image~\cite{goh2017chemnet}, string~\cite{GmezBombarelli2018AutomaticCD}, and sphere~\cite{boomsma2017spherical}. For example, Goh et al.~\shortcite{goh2017chemnet} converted molecular diagrams into 2D RGB images and proposed the ChemNet for the prediction. However, this grid-like transformation usually caused information loss of the molecules which lied in non-Euclidean space, where the internal spatial and distance information of atoms were not fully considered \cite{bronstein2017geometric}. Therefore, some works operated the molecule as a atom graph and developed graph convolutional neural networks for the property prediction~\cite{schutt2017quantum,Gilmer2017NeuralMP}. For instance, Schutt et al.~\shortcite{schutt2017quantum} proposed the deep tensor neural network that captured the representation of each atom node in molecules. Shang et al.~\shortcite{shang2018edge} further introduced attention mechanism for characterizing the edge information to improve the prediction.

Our work improves the previous studies as follows. First, we propose the multilevel graph network to directly model the multilevel quantum interactions of molecules from hierarchical perspectives (i.e., atom-wise, pair-wise, triple-wise, etc), which developed the graph modeling for molecular property prediction. Second, our work could pass the interaction information level-by-level, which benefits more practical scenarios, i.e., generalizability of limited data and transferability of unbalanced data.



%\textbf{Convolutional Neural Networks.}\ Compared to former ML models, one crucial superiority of Convolutional Neural Networks (CNNs) is that automatic feature engineering could replace hand-craft work. Along this line, many previous works dedicated efforts to solve the problem with CNNs. However, unlike the grid-like data in computer vision, most data including molecules to be studied in natural sciences lie in non-Euclidean domains, e.g., graphs. Considering that, some of the CNN-based models adapt molecules to grids structures such as image \cite{goh2017chemnet}, string \cite{GmezBombarelli2018AutomaticCD}, and sphere \cite{boomsma2017spherical}.
 
%While these methods tend to achieve better result comprehensively than former ML models, they are not capable of utilizing the structural and spatial information of data amply due to the loss of information in representing molecules as grid-like data. For instance, converting raw data to 2D images leads to the loss of 3D information and the data in the form of string lacks distance details between atoms.  

%In contrast to the normal CNNs, some models generalized CNNs to the graph-like data. Numerous Graph Convolutional Neural Networks (GCNNs) redefined appropriate convolutional and pooling operators for high-dimensional data in non-Euclidean space \cite{bronstein2017geometric}.
 
%\citeauthor{duvenaud2015convolutional} introduced a CNN that operates directly on graph to compute a fingerprint vector of the entire molecule. On the contrary, \citeauthor{schutt2017quantum} developed the Deep Tensor Neural Network (DTNN) to learning latent representation for each node. Then, this model predicts the energy contributions from each atom and sum them to get final result\cite{schutt2017quantum}. In their follow-up work \cite{schutt2017schnet}, they designed a continuous-filter convolutional layer to move beyond grid-bound data. Similar architectures were also used in protein interface prediction \cite{fout2017protein} with the inclusion of learning edge representations. \citeauthor{shang2018edge} introduced the attention mechanism to GCNN by characterizing edges in terms of multiple relationships , but this model needs extra information such as bond type, and aromaticity \cite{shang2018edge}. Many of GCNNs models could be reformulated to a common framework called Message Passing Neural Network (MPNN) which is composed of a message passing phase and a readout phase \cite{Gilmer2017NeuralMP}.  

%Despite the decent performance these models achieved, none of them considered the multi-level interactions in the molecules.





==> 4_technic.tex <==

\section{Multilevel Graph Convolutional Network}
In this section, we first formally introduce the molecular property prediction problem. Then we describe our Multilevel Graph Convolutional Network in detail.


\subsection{Problem statement}
Given a molecule, it is natural to represent it as graphs without the loss of information, where vertices represent atoms and edges represent chemical bonds. Thus, a molecule is denoted by $\mathcal{G} \langle \mathcal{V}, \mathcal{E} \rangle$, and in the setting of molecular structure, $\mathcal{V}$  is a set of atoms with $|\mathcal{V}|=N$. We regard the graph as a complete undirected graph following the assumption that every atom has the interactions with others so that the set of edges satisfies that $|\mathcal{E}| = N(N-1)/2 $. Here each $\mathcal{E}$ contains two kinds of information, namely edge type and spatial information, respectively. Our target is to construct a regressor to predict the properties of molecules. Formally, we can define the problem as:  
\begin{small} \begin{equation}
    g(f(\mathcal{G})) = y,  
\end{equation} \end{small}  
where $y$ is the target property to predict and the middle function $f:\mathcal{G}\rightarrow \mathbb{R}^{N\scriptsize{\times}  D}$ is used to learn representations of atoms. Then $g$ converts the obtained features to final result.   

The multilevel interactions widely exist in the graph structures. In the field of molecule, physical experts design the different symmetry functions to describe the atomic environment by considering the interactions at varied levels \cite{behler2014representing}. Inspired by this idea, we model quantum interactions in molecules by representing the interactions between two, three, and more atoms level by level to demystify the complexity of molecular interactions. In the next subsection, we will introduce our Multilevel Graph Convolutional Network (MGCN) in detail.   



% Furthermore, the multi-level interactions widely exist in the graph structures. In the field of molecules, the different symmetry functions that applied to describe the atomic environment in physics take the multi-level information into consideration as well \cite{behler2014representing}. In our MGCN model, we extend the representations of nodes to a higher order after each interaction layer. 

\subsection{Network Architecture}  
  
\begin{figure*}[tb]
\centerline{\includegraphics[width=16.5cm]{figures/arch}}
\caption{The architecture of the entire MGCN.} 
\label{network}
\end{figure*}


\textbf{Overview.}\ The entire architecture could be split into three parts in a high-level discussion except for the input. The initial input is a graph which consists of a list of atoms and a Euclidean distance matrix of the molecules. The pre-processing part includes embedding layer and Radial Basis Function (RBF) layer. The embedding layer generates atom and edge embeddings while Radial Basis Function (RBF) layer converts the distance matrix to a distance tensor. The next part of MGCN are several interaction layers that aim to learn different node representations in different levels. The last phase is the readout layer that outputs the final result. 

\textbf{Embedding Layer.}\ Atoms and bonds are the basic elements in a molecule. Thus, to model interactions with as less information loss as possible, we present an embedding layer to directly embed vertices and edges of a graph into vectors.
%In our model, the embedding layer generates the initial embeddings of vertices and edges. 
Each atom in a molecule is represented as a vector $\bm{a}^0\scriptsize{\in} \mathbb{R}^D$ initially. Therefore, the vertices in the entire molecular are denoted as a matrix $ A^0 \scriptsize{\in} \mathbb{R}^{N\scriptsize{\times}  D}$ and $\bm{a}^0_i$ indicates the atom embedding of $i$-th atom in a molecule. The atoms that have the same number of protons in their atomic nuclei share the same initial representation which is called the atom embedding here. Taking \ce{CH2O2} as an example, there are five atoms and different kinds of atoms are labeled with different colors in the input part of Figure \ref{network}. After the process of embedding layer, we get a $5 \scriptsize{\times}  D$ matrix and the rows that are related to the atoms of the same type share the same value. The atom embeddings of all chemical elements are generated randomly before training. The initialization of pair-wise embeddings $\bm{e}\scriptsize{\in} \mathbb{R} $ is similar to atom embeddings (see the preprocess part of Figure \ref{network}). Thus we get $E\scriptsize{\in} \mathbb{R}^{N \scriptsize{\times}  N \scriptsize{\times}  D}$, and the edges connecting the same set of atoms have the same initial edge embedding. Specifically, $\bm{e}_{ij}$ indicates the edge embedding of the bond between $i$-th atom and $j$-th atom. The representations generated by the embedding layer are only related to the inherent property of isolated atoms and bonds. The interaction terms are modeled in later subnetwork.  

% \begin{figure}[tb]
% \centerline{\includesvg[width=8cm]{figures/emb3.svg}}
% \caption{The process of generating initial embeddings}
% \label{input}
% \end{figure}


\textbf{Radial Basis Function Layer.}\ The spatial information influences the degree of interactions between nodes and we use the RBF Layer to convert these information to robust distance tensors for further utilization. First of all, we reform the raw coordinates of atoms to distance matrix to remove the disturbance of selection of coordinate frame. Secondly, Radial Basis Functions are applied to convert the distance matrix to a distance tensor.

% The RBF layer converts the spatial information to distance tensors. First of all, while the raw data provides coordinates of atoms, a pre-processing that converts coordinates to distance matrix could remove the disturbance of the selection of coordinate frame. This could enhance the generability of our model. Secondly, 
% Equally important advantages of using distance matrix are rotating invariance and translation invariance that are essential properties of CNNs \cite{bronstein2017geometric}. 

RBF is a widespread kernel method which originally was invented to generate function interpolation \cite{broomhead1988radial}. Its variant was proved to be advantageous to create fingerprint-like descriptor of molecules \cite{Li2018DeeperII}. Here we use RBF to spread the 2D inter-atomic distance matrix to a 3D representation. Given a set of $K$ central points $\{ \mu_1,\dots,\mu_K \}$, the single data point $x$, namely one pair-wise distance in the molecule, will be processed as:   

\begin{small} \begin{equation} 
	\mathit{RBF}(x) = \mathop{\frown}\limits_{i=1}^{K}\mathrm{h}(\|x-\mu_i\|). 
\end{equation} \end{small}


\noindent Here the notation $\frown$ means concatenation, and we take Euclidean distance as the norm. As for radial basis function $\mathrm{h}$, we take Gaussian $\exp(-\beta\|x-\mu_i\|^2)$ following the suggestion in \cite{schutt2017schnet} to avoid the long plateau on the initial phases of the training procedure. $k$ central points are picked evenly in the range from the shortest to the longest edge among the entire dataset. Therefore all distances in the dataset will be covered. 

Through the non-linear transformation, the representations of distances between nodes become more robust. Furthermore, more additional interpretation is introduced by radial basis function layer than simple multi-layer perceptron. After the RBF layer, we create the pair-wise distance tensors $D \scriptsize{\in} \mathbb{R}^{N \scriptsize{\times}  N \scriptsize{\times}  K}$, and $d_{ij}$ denotes the distance tensor between $i$-th atom and $j$-th atom.


% \textbf{Dense Layer.}\ The dense layer here is similar to common full-connected layer. Noting that our dense layer includes no activation function in the following text, we use the notation $\mathrm{M}(\bm{x})$ to refer to a dense layer that $\mathrm{M}(x)=W\bm{x} +\bm{b}$ with the input $\bm{x}$ for simplicity.


\textbf{Interaction Layer.}\ To model the multilevel molecular structure with all the conformation and spatial information embedded through previous layers, we construct the interaction layer which is a crucial component of our model. Considering that the quantum interactions in molecules could be transformed at different levels (i.e., atom-wise, atom-pair, atom-triple, etc), our interaction layer is designed by the hierarchical architecture level by level. Specifically, in the $l$-th interaction layer, we define the edge representation $e_{ij}^{l+1}$ and atom representation $a^{l+1}_i$ as:
\begin{small} \begin{equation}\bm{e}^{l+1}_{ij} = \mathrm{h}_{e}(\bm{a}_i^l, \bm{a}_j^l, \bm{e}^l_{ij}), \end{equation} \end{small}  
 \begin{small} \begin{equation}\bm{a}^{l+1}_i = \sum_{\substack{j=1, j\neq i}}^N \mathrm{h}_{v}(\bm{a}^l_j, \bm{e}^l_{ij}, \bm{d}_{ij}), \end{equation} \end{small}  
where $h_e$ is used to update edge representation and $h_v$ is the function that collects the message from the neighbours of the $i$-th atom to generate $\bm{a}_i^{l+1}$. 

With this hierarchical modeling, MGCN could effectively preserve the structure of each molecules and describe its quantum interactions. Specifically, in the first layer, $\bm{a}^0_i$ denotes the atom embedding that show the inherent properties of certain chemical elements. As the forward inference steps, $\bm{a}^1_{i}$ involves the first-order neighbour node and spatial information with the message passed by $\bm{a}^0$, $e$ and $d$. In a similar way, $\bm{a}^2_{i}$ represents the triple-wise interactions, $\bm{a}^3_{i}$ indicates the interactions between four nodes and so on. Therefore, after each interaction layer, we obtain the representations of atoms that reflect the higher-order interactions thanks to decomposition of molecule. 

% In the sequence of interaction phases, we refine the representations of all the atoms by including the higher-order interaction representation. The descriptor constructed by each interaction layer is a building block in the molecular system. Thanks to the multi-level structure and decomposition of atomic interaction, with the aggregation of interaction layers level by level, we obtain more generalizable representations of molecules following quantum-chemical principles. 

The update function $\mathrm{h}_e$ is calculated as:  

 \begin{small} \begin{equation} 
\mathrm{h}_e = \eta \bm{e}^l_{ij} \oplus (1 - \eta)W^{ue} \bm{a}^{l}_i\odot\bm{a}^{l}_j. \end{equation} \end{small}where $\eta$ is the hyper-parameter that controls the influence of former pair-wise information (default value is 0.8). Here $\odot$ and $\oplus$ denote the element-wise dot and plus respectively. In this way, The edge embedding is corrected by the related atomic representations of former interaction layer.

The function $\mathrm{h}_v$ applies the message passing operation to create the atom representation at a higher order. The distance tensor $d_{ij}$ here controls the magnitude of impact in each pair of atoms and the edge embedding $e_{ij}$ provides the extra bond information. Thus, it combines the information of nodes, edges, and space, more formally:  
 \begin{small} \begin{equation}
\mathrm{h}_v = \sigma(W^{uv} ( \mathrm{M}^{fa}(\bm{a}^l_j) \odot \mathrm{M}^{fd}(\bm{d}_{ij}) \oplus \mathrm{M}^{fe}(\bm{e}_{ij})), 
\end{equation} \end{small}
where $\sigma$ is a tanh activation function, $W^{uv}$ is a weight matrix. The notation $\mathrm{M}(\bm{x})$ refers to a dense layer that $\mathrm{M}(x)=W\bm{x} +\bm{b}$ with the input $\bm{x}$ for simplicity. $\mathrm{M}^{fa}$,$\mathrm{M}^{fd}$,$\mathrm{M}^{fe}$ are dense layers here.%TO DO y=Wx+b the use of b  



\textbf{Readout Layer.}\ After the interaction layers, we get atom representations at different levels. In the last phase, we construct a readout layer to make the final prediction utilizing these features more clearly.   

First of all, we aggregate the various atom representations to obtain the final vertex feature map as following:  

 \begin{small} \begin{equation}
\bm{a}_i = \mathop{\frown}\limits_{k=0}^{T}\bm{a}_i^k, 
\end{equation} \end{small}  

\noindent where $T$ indicates the number of interaction layers and $\mathop{\frown}$ means concatenation.    

Secondly, we need to predict the property of molecule with the multilevel representations of each atoms. Fortunately, the molecular properties satisfy additivity and locality. For example, to predict the energetic property, we can model potential energy surfaces as follows \cite{behler2014representing,cubuk2017representations}:  

 \begin{small} \begin{equation}
E=\sum_{i}^{N}\sum_{j}^{N}E_{ij}, 
\end{equation} \end{small} 

\noindent where $E$ is the total energy and $E_{ij}$ indicates the part of energy related to the bond between $i$-th and $j$-th atom ($i\neq j$). Besides, $E_{ii}$ could be regarded as the partial energy that mapped to $i$-th atom. Along this line, we can process the representations separately and then sum them up:   
 \begin{small} \begin{equation}
\hat{y} =\sum_{i=1}^N W^{r^a_{2}}\sigma(\mathrm{M}^{r^a_{1}}(\bm{a}_i)) +  \mathop{\sum\limits_{i=1}^N\sum\limits_{j=1}^N}\limits_{i\neq j} W^{r^e_{2}}\sigma(\mathrm{M}^{r^e_{1}}(\bm{e}_{ij})), 
\end{equation} \end{small}    
\noindent where $\sigma$ is the activation function, more specifically, the softplus function. The former term refers to the contribution of quantum interactions that mapped to each atom. Additionally, the latter term denotes the edge-related contribution that can not be mapped to single particle. Since the atom-related interactions account for vast majority of molecular interactions, the latter term is nuanced. Therefore, when the amount of data is small, we tend to ignore the latter term.


% A simple model that consists of two node-wise dense layers is utilized as the readout layer here:  

%  \begin{small} \begin{equation}\hat{y} = \sum_{i=1}^N W^{r_2}\sigma(\mathrm{M}^{r_1}(\bm{a}_i)). \label{eq:readout1} \end{equation} \end{small}  

%   In the model that trained on the ANI-1 dataset which is much hard to fit, we feed the edge representations $e_{ij}$ to the readout layer as well:  

%  \begin{small} \begin{equation}\hat{y} =\sum_{i=1}^N W^{r^a_{2}}\sigma(\mathrm{M}^{r^a_{1}}(\bm{a}_i)) +  \mathop{\sum\limits_{i=1}^N\sum\limits_{j=1}^N}\limits_{i\neq j} W^{r^b_{2}}\sigma(\mathrm{M}^{r^b_{1}}(\bm{e}_{ij})). \end{equation} \end{small}  
% The meanings of notations we used here is similar to \eqref{eq:readout1}, we process the node and edge features separately and sum them up.  

 To train this model, we use the Root-Mean-Square Error (RMSE) as our loss function: 
  \begin{small} \begin{equation}
     \ell(\hat{y},y)=\sqrt{|\hat{y}-y|^2},
 \end{equation} \end{small}  
 where $\hat{y}$ denotes the predictive value and $y$ is the true value. 

% \textbf{Summary.}\   In brief, the architecture mentioned above could be split into three parts in a high-level discussion. The first part, including embedding layer and RBF layer, converts the raw data to the distance tensor and the initial representations of atoms and edges. Several interaction layers make up the second part which generates the atom representations of different levels.  In the final part, we make the prediction of properties with the representations learned in the former network.

\subsection{Discussion on MGCN} 

\textbf{Generalizability.}\   
In the field of chemistry, the set of all possible molecules in unexplored regions is called chemical space. One of the famous chemical space project \cite{Ruddigkeit2012EnumerationO1} collected 166.4 billion molecules while merely 134k samples of them were labeled \cite{ramakrishnan2015many}. Therefore, the generalization ability of enabling accurate prediction with the limited dataset is indeed essential in our task.

In the design of our model, we decide to use the distance tensors $D$ as the form of spatial information instead of coordinates of atom. Accordingly, MGCN enforces rotation and translation invariance. Henceforth, the representation learned by MGCN is more general and would not be confused with the same molecule in different orientations.  

Moreover, we perform element-wise operations in interaction layers (equation(5) and (6)) to generate representations and process the representations of each atom  respectively. Under those circumstances, the prediction made by our model is irrelevant to sequence of atoms. The index invariance enhances the generalization ability of MGCN.

Additionally, we utilize some normalization techniques such as dropout to prevent overfitting, which also benefits generalizability of our model.

In brief, our model is generalizable which is particular important for molecular property prediction where the amount of training data is limited.

\textbf{Transferability.}\ Since the expensive computational cost is a critical bottleneck which limits capabilities to calculate the properties of large molecules, most open data are small and medium molecules and the amount of large molecules is small. Therefore, the ability of transferring the knowledge learned from small molecules to larges ones could help us deal with the data-hungry of big molecules.  

The atom/edge embeddings generated by embedding layer are only in regard to the type of atoms and edges and irrelevant to the specific molecular structure and 
spatial information. As a result, the chemical-domain knowledge learned in the embeddings is universal in the molecular system no matter small or large molecules. Then, in our mulitilevel phase, we use the embeddings to generate the representation in deeper level, e.g., pair-wise and triple-wise. Although small and large molecules are different in the distribution of atoms and bonds, their interactions in different levels are similar. Consequently, with the general embeddings and similar interaction mechanism, MGCN could infer the higher-level representations to predict property and maintain a certain accuracy. Therefore, our model that trained on the small molecules could obtain competitive performance in the prediction of larger molecules.

Rather than applying the model trained on small molecules to big molecules directly, another way to transfer the knowledge is using pre-trained embeddings. To train a model in large molecules, we could initialize this model with the atom and edge embeddings of another model that was trained on small molecules. The pre-trained embeddings could speed up the convergence and improve the accuracy, because the domain knowledge in embeddings learned from small molecules is still meaning suitable to big molecules.

Along this line, this model is capable of transferring the knowledge of small molecules to large molecules and tackle the structural shortage of data.

\textbf{Time Complexity.}\ 
The time complexity of our MGCN model is $\mathcal{O}(N^2_a)$ since the calculation of $h_e$ and $h_v$ (equation (5) and (6)) are independent of molecular size. Here $N_a$ indicates the number of atoms in a molecule.


 
 
 
 

==> 5_experiments.tex <==

\section{Experiments}

We conduct experiments to demonstrate the effectiveness of MGCN from various aspects: 1) predictive performance; 2) the effectiveness of multilevel structure; 3) the validation of generalizability; 4) the verification of transferability; 5) the influence of varied number of interaction layers.


%To evaluate our method, we ran a series experiments from various aspects: 1) overall predictive performance; 2) the effectiveness of our multilevel structure; 3) the validation of generalizability; 4) the verification of transferability; 5) the influence of varied number of interaction layers. 

\subsection{Datasets}



\textbf{QM9.}\ The QM9\footnote{http://www.quantum-machine.org/datasets/\#qm9} dataset \cite{ramakrishnan2014quantum} is perhaps the most well-known benchmark dataset which contains  134k equilibrium molecules with their 13 different properties. All of the relaxed geometries and properties for all the 134k molecules are calculated by DFT. The DFT error is the empirical inaccuracy estimation of DFT based approaches \cite{faber2017prediction}. The QM9 dataset also provides the chemical accuracy which is generally accepted by the chemistry community as a relatively ideal accuracy. 
% TODO the supplementary materials "More details about the QM9 dataset are provided in the supplementary materials."


% Taprod in the supplvidet ble generaymenaset ted by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[tbp]
\centering
\footnotesize
 \setlength{\tabcolsep}{1.5 mm}
\renewcommand\arraystretch{1.5}

\caption{Predictive accuracy of different models in QM9}
\begin{threeparttable}

\begin{tabular}{lrrrrrrrrrrrrr}
    \toprule
           Properties & \multicolumn{1}{l}{$U_0$} & \multicolumn{1}{l}{$U$} & \multicolumn{1}{l}{$G$} & \multicolumn{1}{l}{$H$} & \multicolumn{1}{l}{$C_v$} & \multicolumn{1}{l}{ $\varepsilon_{\text{HOMO}}$} & \multicolumn{1}{l}{$\varepsilon_{\text{LUMO}}$} & \multicolumn{1}{l}{$\Delta \varepsilon$} & \multicolumn{1}{l}{$\omega_1$} & \multicolumn{1}{l}{ZPVE} & \multicolumn{1}{l}{$\langle R^2 \rangle $} & \multicolumn{1}{l}{$\mu$} & \multicolumn{1}{l}{$\alpha$} \\
           Unit & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{cal/molK} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{$\text{cm}^{-1}$} & \multicolumn{1}{l}{eV} & \multicolumn{1}{l}{$\text{Bohr}^2$} & \multicolumn{1}{l}{Debye} & \multicolumn{1}{l}{$\text{Bohr}^3$} \\
    \midrule
    
    
    DFT Error & 0.1    & 0.1    & 0.1    & 0.1    & 0.34   & -      & -      & -      & 28     & 0.0097 & -      & 0.1    & 0.4 \\
    Chemical Acc. & 0.043  & 0.043  & 0.043  & 0.043  & 0.05   & 0.043  & 0.043  & 0.043  & 10     & 0.00122 & 1.2    & 0.1    & 0.1 \\
    \midrule
    \midrule
    RF+BAML & 0.2000  & -      & -      & -      & 0.451  & 0.1070  & 0.1180  & 0.1410  & 2.71   & 0.01320  & 51.10  & 0.434  & 0.638  \\
    KRR+BOB & 0.0667  & -      & -      & -      & 0.092  & 0.0948  & 0.1220  & 0.1480  & 13.20  & 0.00364  & 0.98   & 0.423  & 0.298  \\
    KRR+HDAD & 0.0251  & -      & -      & -      & 0.044  & 0.0662  & 0.0842  & 0.1070  & 23.10  & 0.00191  & 1.62   & 0.334  & 0.175  \\
    GG     & 0.0421  & -      & -      & -      & 0.084  & 0.0567  & 0.0628  & 0.0877  & 6.22   & 0.00431  & 6.30   & 0.247  & 0.161  \\
    enn-s2s & 0.0194  & 0.0194 & 0.0168 & 0.0189 & 0.040  & 0.0426  & 0.0374 & 0.0688 & 1.90   & 0.00152  & 0.18   & \textbf{0.030} & 0.092  \\
    DTNN   & 0.0364  & 0.0377 & 0.0385 & 0.0357 & 0.089  & 0.0982  & 0.1053  & 0.1502  & 4.23   & 0.00312  & 0.30   & 0.257  & 0.131 \\
    SchNet & 0.0134  & 0.0189 & 0.0196 & 0.0182 & 0.067  & 0.0507  & \textbf{0.0372}  & 0.0795  & 3.83   & 0.00172  & 0.27   & 0.071  & 0.073  \\
    MGCN   & \textbf{0.0129} & \textbf{0.0144} & \textbf{0.0146} & \textbf{0.0162} & \textbf{0.038} & \textbf{0.0421} & 0.0574  & \textbf{0.0642}&\textbf{1.67} & \textbf{0.00112} & \textbf{0.11} & 0.056  & \textbf{0.030}  \\
    \bottomrule
    
    \end{tabular}


\end{threeparttable} 


\label{qm9}%
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[htbp]
  \centering
  \caption{Predictive accuracy of different models in ANI-1}
    \begin{tabular}{lrrrr}
    \toprule
    Methods & \multicolumn{1}{l}{DTNN} & \multicolumn{1}{l}{SchNet} & \multicolumn{1}{l}{MGCN}  \\
    \midrule
    
    MAE    & 0.113  & 0.108   & \textbf{0.078} \\
    \bottomrule
    \end{tabular}%
  \label{ani}%
\end{table}%

\textbf{ANI-1.}\ The ANI-1\footnote{https://www.nature.com/articles/sdata2017193} dataset provides access to the total energies of 20 million off-equilibrium molecules which is 100 times larger than QM9.


\subsection{Experimental Setup}  
 
We use mini-batch stochastic gradient descent (mini-batch SGD) with the Adam optimizer \cite{Kingma2014Adam} to train our MGCN. The batch size is set to 64 and the initial learning rate is 1$e^{-5}$. For all 13 properties of QM9, we pick 110k out of 130k molecules randomly as our training set that accounts for about 84.7\% of the entire dataset. With the rest of the data, we choose half of them as the validation set and the other half as the testing set. As for the much larger ANI-1, we randomly choose 90\% samples for training, 5\% samples for validation and 5\% for testing. We select Mean Absolute Error (MAE) as our evaluation metrics for the convenience of comparison with baselines \cite{faber2017prediction}.

\subsection{Baselines}  

We compare our model with the 7 baseline methods that could be categorized into two groups.   

The first group consist of 3 traditional ML models using hand-engineered features derived from the molecular literature \cite{faber2017prediction,huang2016communication,hansen2015machine}. These ML models include Random Forest (RF) and Kernel Ridge Regression (KRR). The hand-craft features include Bag of Bonds (BOB), Bond-Angle Machine Learning (BAML) and "Projected Histograms" (HDAD). We imply the combination of X regressor and Y representation with the notation X+Y. Thus, these three baselines are denoted by RF+BAML, KRR+BOB, KRR+HDAD. These models achieve the best performance in the prediction of one or more properties among all 30 combinations of regressors and features \cite{faber2017prediction}. 
 
The second group contain 4 deep neural networks. They are gated graph network (GG, \citeauthor{kearnes2016molecular} \citeyear{kearnes2016molecular}), edge neural network with set-to-set (enn-s2s, \citeauthor{Gilmer2017NeuralMP} \citeyear{Gilmer2017NeuralMP}), deep tensor neural network (DTNN, \citeauthor{schutt2017schnet} \citeyear{schutt2017quantum}) and SchNet \cite{schutt2017schnet}. These models are proved to be competitive in the molecular property prediction. Noting that DTNN and SchNet only provide their experimental results in the prediction of property $U_0$ for the molecules in QM9, thus we complete the rest of the experiments. Besides, all of other numerical results of the baselines are extracted from their works directly.

        


\subsection{Experimental Results}
\textbf{Predictive performance.}\ We compare our model with the baseline models mentioned above in two datasets. In Table \ref{qm9}, we provide the MAE of baselines and our approach as well as DFT error and chemical accuracy for all 13 properties. Table \ref{ani} shows the performance comparison in ANI-1.

As illustrated in Table \ref{qm9}, MGCN gets the best performance in 11 out of 13 properties, and 11 of them exceed the chemical accuracy. Our model is able to improve the performance upon state-of-the-art. Another observation is that the deep neural networks (GG, enn-s2s, DTNN, SchNet and MGCN) outperform the models that using hand-craft features comprehensively. 
In the experiment in ANI-1, we choose the state-of-the-art models (DTNN and SchNet) as comparison. As shown in Table \ref{ani}, the accuracies in ANI-1 is lower than in QM9, and there are possible two reasons. First, the force in equilibrium molecules of QM9 is negligible, while in off-equilibrium molecules of ANI-1, this factor increases the complexity of quantum interactions. Second, the 100 times larger size of ANI-1 than QM9 makes it more difficult to ﬁt. Even though, our model still achieves satisfactory accuracy and outperform other methods.

In brief, our model attains the best performance benefiting from the mulitilevel interaction modeling, and the results prove that our model could handle both equilibrium and off-equilibrium molecules and is capable to fit the large dataset. Considering that most previous work have no experiment in the ANI-1 dataset, we chose QM9 as our default dataset in the rest of our experiments.  
% Given that the enn-s2s model outperformed the MGCN in $\varepsilon_{\text{LUMO}}$, $\Delta\varepsilon$ and $\mu$, one of the reason is that these properties do not follow the additivity so much and the second reason is that enn-s2s model benefits from extra data like the bond type. 
% However, it is worth noting that there is no guarantee that these models can meet the same performance on the ground-truth data due to the relatively low precision of the QM9 dataset itself. 

% TODO comparision with DFT in tim comsuing

% \textbf{ANI-1 Results.}  MGCN achieves a quite fair accuracy: the first model predicts energies with 0.109 eV MAE and the error of the second model is 0.07758. As a comparison, we applied DTNN and SchNet in the ANI-1 and their MAE is 0.113, 0.108 respectively. The results prove that our model could handle both stable and off-equilibrium molecules and is capable to fit the large dataset.



\begin{figure}[tb]
	
    \centerline{\includegraphics[width=8.5cm]{figures/maesize}}

    \caption{MAE of prediction in different size molecules.}
    \label{maeatom}
\end{figure} 


 \textbf{Effectiveness of multilevel interactions.}\ In the molecular system, with the increase of the number of atoms in a molecule, the complexity of quantum interactions will grow exponentially. In consequence, it is much harder to model the interactions of molecules if the size of them is larger.
 

 Figure \ref{maeatom} shows the MAE of predictions as the function of the number of atoms. We select the state-of-the-art work SchNet as a comparison for better illustration. Four representative and prevalent properties ($\mu$, $\varepsilon_{\text{HOMO}}$, $U$, $Cv$) are picked in this experiment. The dotted horizontal line in each subplot is the chemical accuracy of each property. Figure \ref{maeatom} shows that MGCN assesses more accurate and stable performance than SchNet. Furthermore, as the number of atoms increases, the advantage of MGCN becomes more apparent due to the multilevel modeling. Our model simplifies the interactions by dividing them into different levels and represent them respectively using the mulitilevel structure and decomposition of molecular quantum interactions. Along this line, our model performs better comparatively when the number of atoms increases. In addition, the significant fluctuations appearing in the front and end of the curves derive from the lack of molecules that contain less than 10 atoms or more than 24 atoms in dataset.  
 
 To investigate this further, we construct a control model that blends all levels of interactions in a single embedding rather than construct representation level by level. Taking the prediction of $U$ property for example, the result of this model is not as well as our MGCN with an MAE of 0.03683 on average. It implies the molecular representations modeled by multilevel interaction layers are more robust, which validates the effectiveness of our multilevel modeling.
 
 
%  We select molecules with  properties from the QM9 dataset to show the MAE on the QM9 dataset depending on the size of molecule. Since result in the property $U_0$ is similar to the other three energies, $U$, $G$, $H$, we merely choose $U_0$ to make the observation. We omit the properties $\varepsilon_{\text{LUMO}}$ and $\Delta \varepsilon$ for the same reason. Take Figure  \ref{maeatom} as an illustration, the dotted horizontal line in each subplot is the chemical error of each property. In most of the properties, and there are no significant differences in the MAE of diverse size molecules that contain 10 to 26 atoms. We observe that the molecules with less than 9 atoms have higher errors relatively due to the lack of smaller molecules in the dataset (see Figure  \ref{atomcount}) that makes it hard to learn the interaction in a smaller chemical environment. The same argument applies to the increase of error when predicting the molecules with more than 26 atoms. 

\begin{table}[tbp]
\centering
\caption{Performance comparison in varied size training set}
\begin{tabular}{rrrrr}
    \toprule

    \multicolumn{1}{l}{N} & \multicolumn{1}{l}{SchNet} & \multicolumn{1}{l}{DTNN} & \multicolumn{1}{l}{enn-s2s} & \multicolumn{1}{l}{MGCN} \\
    \midrule
    \midrule
    50,000 & 0.0256 & 0.0408 &  0.0249& \textbf{0.0229} \\
    100,000 & 0.0147 & 0.0364 & - & \textbf{0.0142} \\
    110,462 & 0.0134 & -      & 0.0194 & \textbf{0.0129} \\
    \bottomrule

\end{tabular}%

\label{size}%
\end{table}%

 %\footnote{As reported in \cite{Gilmer2017NeuralMP}. The model was trained on 58k training samples vs 50k used in our experiments.} 

\begin{figure}[tpb]
    \centerline{\includegraphics[width=8.5cm]{figures/GT}}
    \caption{$a$(left). Performance comparison in the training set with different size. $b$(right). Predictive performance of models with different number of interaction layers.}
    \label{interaction}
\end{figure}

\textbf{Generalizability.}\ The potential molecules in chemical space is numerous extra, but the amount of labeled data is quite small \cite{schutt2017quantum}. Due to the limitation of the magnitude of existing datasets, the ideal model should be able to perform well even trained with a small amount of data. Thus, the generalizability is another essential aspect to evaluate these models.  

We train our model in three training sets with the different size that consist of 50k, 100k and 110k samples respectively and test them in the same test set that contains 10k molecules. In addition to the three baselines mentioned above (DTNN, SchNet, enn-s2s), the ensemble model of five enn-s2s models is also listed in the comparison. In Table \ref{size}, the MGCN gets the lowest MAE in three training sets. Regarding that the readout phase of MGCN and SchNet are similar, the representation of molecular learned by MGCN is more generalizable when the accessible data is smaller thanks to the modeling of multilevel interactions.   

\textbf{Transferability.}\ As mentioned before, the data in existing datasets are unbalanced. For instance, relative large molecules that contain more than 20 atoms account for merely 20.7\% of total amount in QM9 and only occupy 8.5\% in ANI-1. Therefore, the transferability is quite important to an approach.  

We conduct experiments to validate the transferability of MGCN. Specifically, we sample 50k small and 50k large molecules from QM9 respectively. As shown in Figure \ref{interaction}.$a$, there are four experimental settings. The first two models are trained and tested on the small and large molecules respectively (noted by "Small" and "Large"). The latter two approaches are different ways to transfer the knowledge. The "Develop" denotes the develop model which is trained on the small molecules and applied to the large ones directly. The last model (labeled with "Pre-train") utilizes the embeddings learned on the small molecules as initialization, and then refine itself during the training on the large molecules. 

Figure \ref{interaction}.$a$ illustrates the performance of MGCN in four settings. In the first place, The MAE of small molecules is lower relatively due to the higher complexity of large molecules. Secondly, we observe that as we feed in more small data, the MAE of develop model keeps decreasing. The performance is fairly decent because we did not feed any large molecules to this model. The numerical results show that our model is capable to learn knowledge from small data and then transfer them to larger molecules. Thirdly, the pre-trained model outperforms all of other models when the size of training set is small with the universal domain knowledge learned before. This technique helps address the structural shortage of data.

 
% \begin{figure}[tb]
%     \centerline{\includesvg[width=7.5cm]{figures/trans.svg}}
%     \caption{Performance of models that trained on the smaller molecules.}
%     \label{trans}
% \end{figure}


\textbf{Influence of interaction layers.}\ In DFT, physicists usually use 4 to 5 different empirical symmetry functions for molecular property prediction. Each symmetry could be mapped to the interaction layer in each level. Figure \ref{interaction}.$b$ shows the relationship between the number of interaction layers and the MAE of property $U_0$. We randomly pick 50k molecules as our training set and test on remaining data. As Figure \ref{interaction}.$b$ illustrates, too many or few interaction layers could cause higher MAE. The network with less than 4 interaction layers does not have enough capacity to learn the representations of molecules and using the deeper model that contain more than 5 interaction layers will widen the generalization gap. The empirical results indicate that four is the best number of interaction layers which conform to the number of symmetry functions mentioned previously. 

\textbf{Summary.}\ Through the experiments, MGCN shows the superiority of incorporating multilevel modeling of molecular interactions. Moreover, the experimental results prove that our model is generalizable and transferable. Besides, in theory, the time complexity of MGCN is $\scriptsize{\mathcal{O}(N^2)}$ compared with $\scriptsize{\mathcal{O}(N^3)}$ of DFT. Experimentally, with the same setting (a single core of a Xeon E5-2660), our model spends $\scriptsize{2.4\scriptsize{\times}10^{-2}}$ second predicting the property of one molecule, which is nearly $\scriptsize{1.5\scriptsize{\times}10^{5}}$ times faster than DFT. 

%  it takes nearly $\scriptsize{3.6\scriptsize{\times}10^3}$ seconds to finish the calculation on a single medium size molecule in QM9 using a single core of a Xeon E5-2660(2.2GHz) \cite{Gilmer2017NeuralMP}. With the same CPU setting, the time cosuming of MGCN is only $\scriptsize{2.4\scriptsize{\times}10^{-2}}$ second per molecule. Furthermore, a single GPU (Tesla K80) could reduce the time to $\scriptsize{4.1\scriptsize{\times}10^{-4}}$. Generally speaking, our model is nealry $\scriptsize{10^5\scriptsize{\sim}10^6}$ times faster than DFT.



==> 6_conclusion.tex <==

\section{Conclusion}

In this paper, we introduced a Multilevel Graph Convolutional Network (MGCN) for molecular property prediction. The well-designed model utilized the multilevel structure in molecular system to learn the representations of the quantum interactions level by level, and then made prediction with overall interaction representation. The experimental results on two prevalent datasets demonstrated the competency of our approach. Furthermore, our model was proved to be generalizable and transferable.  

We believe the future research should concentrate efforts on enhancing the generalization of the atom representation because the predictive accuracy is quite high in small samples and it is tough to obtain the dataset of sufficient large molecules. 
% which is an extended CNN architecture designed to process graph-structured data. MGCN models the quantum molecular interactions from the perspective of multiscale structure. The representations of molecules generated by MGCN is translation invariant, index invariant, generalizable and transferable. Our experiments show that MGCN achieves the state of the art accuracy in two widely used datasets. Moreover, numerical results prove the transferability and generalizability of our model. 
